Self-Distillation Bridges Distribution Gap in Language Model Fine-Tuning

The surge in Large Language Models (LLMs) has revolutionized natural language processing, but fine-tuning them for specific tasks often encounters challenges in balancing performance and preserving general instruction-following abilities. In this paper, we posit that the distribution gap between task datasets and the LLMs serves as the primary underlying cause. To address the problem, we introduce Self-Distillation Fine-Tuning (SDFT), a novel approach that bridges the distribution gap by guiding fine-tuning with a distilled dataset generated by the model itself to match its original distribution. Experimental results on the Llama-2-chat model across various benchmarks demonstrate that SDFT effectively mitigates catastrophic forgetting while achieving comparable or superior performance on downstream tasks compared to the vanilla fine-tuning. Moreover, SDFT demonstrates the potential to maintain the helpfulness and safety alignment of LLMs. Our code is available at https://github.com/sail-sg/sdft.

==> tables/math.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{lccc}
    \toprule
         \textbf{Method} & \textbf{GSM8K} & \textbf{MultiArith} \\
    \midrule
         Original & 29.42 & 70 \\
         SFT & 31.92 & 76.11 \\
         SDFT & \textbf{34.42} & \textbf{83.89} \\
    \bottomrule
    \end{tabular}
    \caption{Experiments on math reasoning. SDFT has better generalization ability.}
    \label{tab:math}
\end{table}
